A new membership inference attack that spots memorization in generative and predictive models: Loss-Based with Reference Model algorithm (LBRM)

Generative models can unintentionally memorize training data, posing significant privacy risks. This paper addresses the memorization phenomenon in time series imputation models, introducing the Loss-Based with Reference Model (LBRM) algorithm. The LBRM method leverages a reference model to enhance the accuracy of membership inference attacks, distinguishing between training and test data. Our contributions are twofold: first, we propose an innovative method to effectively extract and identify memorized training data, significantly improving detection accuracy. On average, without fine-tuning, the AUROC improved by approximately 40\%. With fine-tuning, the AUROC increased by approximately 60\%. Second, we validate our approach through membership inference attacks on two types of architectures designed for time series imputation, demonstrating the robustness and versatility of the LBRM approach in different contexts. These results highlight the significant enhancement in detection accuracy provided by the LBRM approach, addressing privacy risks in time series imputation models.

==> Dicussion.tex <==
\section{Discussion}
The LBRM (Loss-Based Reference Model) approach stands out in the realm of membership inference attacks due to its innovative use of a reference model \referencemodel to enhance the accuracy of distinguishing between training and test data. This method is particularly relevant in scenarios where the target model \targetmodel is either exclusively trained on private data or fine-tuned with private data after initial training on public data.

One of the key strengths of the LBRM approach is its improved accuracy. By leveraging the R(x) score, the LBRM method consistently outperforms the naive loss approach in terms of performance metrics like AUROC and TPR. For instance, in Scenario 1, the SAITS model's AUROC increased from 0.52 to 0.71, and the AE model's AUROC improved from 0.55 to 0.77. In Scenario 2, the SAITS model's AUROC went from 0.55 to 0.90, and the AE model's AUROC increased from 0.52 to 0.85. These results highlight the significant enhancement in detection accuracy provided by the LBRM approach.

Additionally, the LBRM approach is robust across different scenarios, whether the target model is trained solely on private data or fine-tuned with private data. This versatility makes it a reliable choice for various contexts. Another significant advantage is the minimal overfitting observed in the models, as the reference model \referencemodel and target model \targetmodel are ensured to have similar performance levels. This precaution helps maintain the integrity of the attack and ensures that the observed outcomes are due to the attack methodology rather than artifacts of model training. Furthermore, the effectiveness of the LBRM attack is independent of the threshold \threshold used, making it adaptable to different settings and requirements.

A notable strength of the LBRM approach is its ability to capture small parts of memorized data, not just overfitting. By incorporating a reference model, the LBRM method can detect subtle memorization patterns that might be missed by the naive loss approach. This capability enhances the effectiveness of the attack, making it a more powerful tool for membership inference.

However, the LBRM approach also has its weaknesses. One notable limitation is the dependency on the reference model \referencemodel. The need for a reference model that has comparable performance to the target model \targetmodel can be challenging. If the reference model's performance significantly deviates from the target model, the attack's success rate may be adversely affected. Additionally, the LBRM approach is more complex than the naive loss approach, requiring additional steps to train and evaluate the reference model. This complexity might pose challenges in implementation and computational resources.


